Active Learning of Symbolic NetKAT Automata

NetKAT is a domain-specific programming language and logic that has been successfully used to specify and verify the behavior of packet-switched networks. This paper develops techniques for automatically learning NetKAT models of unknown networks using active learning. Prior work has explored active learning for a wide range of automata (e.g., deterministic, register, B\"uchi, timed etc.) and also developed applications, such as validating implementations of network protocols. We present algorithms for learning different types of NetKAT automata, including symbolic automata proposed in recent work. We prove the soundness of these algorithms, build a prototype implementation, and evaluate it on a standard benchmark. Our results highlight the applicability of symbolic NetKAT learning for realistic network configurations and topologies.

==> Makefile <==
default: draft.pdf

%.pdf: %.tex local.sty
	latexmk -pdf $<

clean:
	latexmk -c
	rm *.bbl notes.pdf draft.pdf

# Script for latex-diff
FILE = draft
DIFF_COMMIT ?= 15ef60cd9b8b75e1f9821b7463267ba68752c300 # tag: submit

THIS_REPO ?= git@github.com:cornell-pl/netkat-learning.git

PAPER_DIR ?= papers/nkl
UNDO_PAPER_DIR ?= ../..

diff:
	rm -rf tmp/diff
	rm -rf tmp/old-src
	mkdir -p tmp/diff/old
	mkdir -p tmp/diff/new
	mkdir -p tmp/diff/delta
	
	make default
	latexpand $(FILE).tex > tmp/diff/new/$(FILE).tex
	cp *.bib tmp/diff/new/
	cp *.sty tmp/diff/new/
	
	git clone --depth=1 $(THIS_REPO) tmp/old-src
	cd tmp/old-src && ( \
	  git fetch origin $(DIFF_COMMIT) && \
	  git checkout $(DIFF_COMMIT) && \
	  cd $(PAPER_DIR) && ( \
	    latexmk -pdf -auxdir=aux $(FILE) && \
	    latexpand $(FILE).tex > $(UNDO_PAPER_DIR)/../diff/old/$(FILE).tex && \
	    cp *.bib $(UNDO_PAPER_DIR)/../diff/old/ && \
	    cp *.sty $(UNDO_PAPER_DIR)/../diff/old/    \
	))
	
	cd tmp/diff/new && ( \
	  latexdiff ../old/$(FILE).tex $(FILE).tex > ../delta/$(FILE).tex && \
	  cp *.bib ../delta/ && \
	  cp *.sty ../delta/ \
	)
	
	cd tmp/diff/delta && ( \
	  (latexmk -pdf -auxdir=aux -interaction=nonstopmode $(FILE).tex || true) \
	)
	
	cp tmp/diff/delta/$(FILE).pdf $(FILE)-diff.pdf

.PHONY: build clean

